Dynamic Stochastic Decoding Strategy for Open-Domain Dialogue Generation

Stochastic sampling strategies such as top-k and top-p have been widely used in dialogue generation task. However, as an open-domain chatting system, there will be two different conversation scenarios, i.e. chit-chat and knowledge-based question answering. In the former situation, responses diversity is essential due to the one-to-many nature in dialogue. The latter, on the other hand, requires less randomness given that stochastic decoding strategy entails the risk of generating incorrect information. As a result, an adaptive and flexible decoding strategy is needed to cope with these two scenarios simultaneously. To this end, we propose the dynamic decoding strategy (DDS), which can adjust the decoding space w.r.t. different contexts. In DDS, both sequence-level and token-level adaptive search can be achieved to adjust the decoding process in a unified framework. Besides, our adaptive algorithm can not only be used during model inference, but it can also be applied during the model training stage to further enhance the performance. Comprehensive experiments indicate that the proposed decoding strategy can consistently improve the performance of pre-trained dialogue models when coupled with four well-used stochastic decoding algorithms.

==> related_work.tex <==
\section{Related Work}
% \subsection{Pretrained Dialogue Models}
% % 重点突出对话预训练模型
% In contrast with plain texts for general language models, massive conversations are used for dialogue generation pre-training.


% \subsection{Decoding Strategies for Natural Language Generation}
% Two widely used deterministic decoding approaches are greedy search and beam search. For Stochastic Decoding Algorithms.
Greedy search is the most basic decoding method, in which the token with the highest likelihood is selected at each step of the generation process. 
The most widely used decoding algorithm in text generation is beam search, a basic breadth-first search algorithm. 
Unfortunately, they naturally suffer from a lack of diversity and often lead to degeneration in open-ended scenarios. Diverse beam search \citep{DBS} is proposed to overcome the lack of diversity in the returned strings. However, it is still deterministic decoding strategy which is not suitable for open-domain chatbot.

Stochastic decoding strategies involve randomness in the generation of sequences. Ancestral sampling \citep{sampling} is the most straightforward sampling method, while temperature sampling \citep{temperature} introduces temperature to shape the probability distribution. In order to mitigate the damage of randomness to quality, some approaches are proposed to truncate the distributions, such as top-$k$ \citep{fan-etal-2018-hierarchical}, top-p \citep{top-p}, and locally typical \citep{typical} sampling, aiming at improving quality while preserving diversity. However, they still can not get rid of the trade-off of quality and variety. Different from them, we propose dynamic decoding strategy to adjust the shape of distributions adaptively, which can further enhance the quality and diversity simultaneously.


